Learning Deep Matrix Representations

We present a new distributed representation in deep neural nets wherein the information is represented in native form as a matrix. This differs from current neural architectures that rely on vector representations. We consider matrices as central to the architecture and they compose the input, hidden and output layers. The model representation is more compact and elegant -- the number of parameters grows only with the largest dimension of the incoming layer rather than the number of hidden units. We derive several new deep networks: (i) feed-forward nets that map an input matrix into an output matrix, (ii) recurrent nets which map a sequence of input matrices into a sequence of output matrices. We also reinterpret existing models for (iii) memory-augmented networks and (iv) graphs using matrix notations. For graphs we demonstrate how the new notations lead to simple but effective extensions with multiple attentions. Extensive experiments on handwritten digits recognition, face reconstruction, sequence to sequence learning, EEG classification, and graph-based node classification demonstrate the efficacy and compactness of the matrix architectures.

==> matrix-abs_sv.tex <==
\begin{abstract}
We present a new distributed representation in deep neural nets wherein
the information is represented in native form as a matrix. This differs
from current neural architectures that rely on vector representations.
We consider matrices as central to the architecture and they compose
the input, hidden and output layers. The model representation is more
compact and elegant \textendash{} the number of parameters grows only
with the largest dimension of the incoming layer rather than the number
of hidden units. We derive feed-forward nets that map an input matrix
into an output matrix, and recurrent nets which map a sequence of
input matrices into a sequence of output matrices. Experiments on
handwritten digits recognition, face reconstruction, sequence to sequence
learning and EEG classification demonstrate the efficacy and compactness
of the matrix-centric architectures.
\end{abstract}



==> matrix-discuss.tex <==
We have introduced a new notion of distributed representation in neural
nets where information is distributed across neurons arranged in a
matrix. This departs from the existing representation using vectors.
Matrix-centric representation is in line with recent memory-augmented
RNNs, where external memory is an array of memory slots \textendash{}
essentially a matrix arrangement. However, in our treatment, matrices
are first-class citizen: neurons in a layer are always arranged in
a matrix. We derive matrix-centric feedforward and recurrent nets,
and propose a method to convert convolutional outputs into a matrix.
We theoretically show that through matrix factorization of weights,
a traditional vector net can be replaced by an equivalent matrix net
when modeling matrix data. This results in much a more compact matrix-centric
net, and benefits from structural regularization. We evaluate our
proposed neural architectures on four applications: handwritten digit
recognition (MNIST), face reconstruction under block occlusion, sequence-to-sequence
prediction of moving digits, and EEG classification. The experiments
have demonstrated that matrix-centric nets are highly compact and
perform better than vector-centric counterparts when data are inherently
matrices.

Matrix-centric representation opens a wide room for future work. Structural
regularization, the loss surfaces and the connection with memory-augmented
RNNs deserve more deep investigations. It might also be useful to
design matrix-centric CNNs, where the receptive fields can be factorized
via the matrix-matrix mapping. Further, as matrix is an effective
representation for graphs, it remains open to apply matrix-centric
nets in these domains.




==> matrix-exp-v2.tex <==
In this section, we experimentally validate the proposed matrix-centric
architectures described in Section.~\ref{sec:Methods}. For all experiments
presented below, our networks use ReLU activation function and are
trained using Adam \cite{kingma2014adam}.  

\subsection{Feedforward Nets on MNIST}

The MNIST dataset consists of 70K handwritten digits of size $28\times28$,
with 50K images for training, 10K for testing and 10K for validation.
For matrix nets, images are naturally matrices, but for traditional
vector nets, images are vectorized into vectors of length $784$.
To test the ability to accommodate very deep nets without skip-connections
\cite{srivastava2015training,pham2016faster}, we create vector and
matrix feed-forward nets with increasing depths. The top layers are
softmax as usual for both vector and matrix nets. We compare matrix
nets with the hidden shape of $20\times20$ and $50\times50$ against
vector nets containing 50, 100 and 200 hidden units.

\begin{figure}
\begin{centering}
\includegraphics[width=0.9\columnwidth]{MNIST-err-mat_vec}
\par\end{centering}
\caption{Test errors of matrix and vector feed-forward nets over MNIST with
depth varying from 5 to 30. Nets trained without Batch-Norm. Best
viewed in color.\label{fig:Test-errors-MNIST-without-BN}}
\end{figure}

We observe that without Batch-Norm (BN) \cite{ioffe2015batch}, vector
nets struggle to learn when the depth goes beyond $20$, as evidenced
in Fig.~\ref{fig:Test-errors-MNIST-without-BN}. The erratic learning
curves of the vector nets at depth 30 are shown in Fig.~\ref{fig: MNIST-vec30},
top row. With the help of BN layers, the vector nets can learn normally
at depth 30 (see the test errors in Fig.~\ref{fig:Test-errors-MNIST-without-BN}),
but again fail beyond depth 50 (see Fig.~\ref{fig: MNIST-vec30},
bottom row). The matrix nets are far better: They learn smoothly at
depth 30 without BN layers (Fig.~\ref{fig:MNIST-mat30}, top). With
BN layers, they still learn well at depth 50 (Fig.~\ref{fig:MNIST-mat30},
bottom) and can manage to learn up to depth 70 (result is not shown
here). These behaviors suggest that matrix nets might exhibit a
form \textit{structural regularization} that simplifies the loss surface,
which is the subject for future investigation (e.g., see \cite{choromanska2015loss}
for an account of vector nets).

\begin{figure}[h]
\begin{centering}
\subfloat[Vector nets\label{fig: MNIST-vec30}]{\includegraphics[scale=0.3]{MNIST-vec-d30,50BN}

}\subfloat[Matrix nets\label{fig:MNIST-mat30}]{\includegraphics[scale=0.3]{MNIST-mat-d30,50BN}

}
\par\end{centering}
\caption{Learning curves of vector and matrix feed-forward nets over MNIST.\textbf{
(a)} \textbf{Left to right:} Vector nets with $50$, $100$, $200$
hidden units. \textbf{(b)}: Matrix nets with $50\times50$ hidden
units. \textbf{Top:} $30$-layer nets without Batch Norm. \textbf{Bottom:}
$50$-layer nets with Batch Norm.\label{fig:MNIST_err_curve}}
\end{figure}

We visualize the weights of the first layer of the matrix net with
hidden layers of $50\times50$ (the weights for $20\times20$ layers
are similar) in Fig.~\ref{fig:MNIST_weights} for a better understanding.
In the plots of $U$ and $V$ (top and bottom left of Fig.~\ref{fig:MNIST_weights},
respectively), the short vertical brushes indicate that some adjacent
input features are highly correlated along the row or column axes.
For example, the digit $1$ has white pixels along its line which
will be captured by $U$. In case of $W$, each square tile in Fig.~\ref{fig:MNIST_weights}(right)
corresponds to the weights that map the entire input matrix to a particular
element of the output matrix. These weights have cross-line patterns,
which differ from stroke-like patterns commonly seen in vector nets.

\begin{figure}[h]
\begin{centering}
\includegraphics[scale=0.5]{MNIST-d30-h50,50-U,V,W}
\par\end{centering}
\caption{The normalized weights of the first layer of the 30-layer matrix feed-forward
net with hidden size of $50\times50$ trained on MNIST. Weights of
other layers look quite similar. \textbf{Top left:} Row mapping matrix
$U$ of shape $28\times50$. \textbf{Bottom left:} Column mapping
matrix $V$ of shape $28\times50$. \textbf{Right:} Each square tile
$i$, $j$ show the weight $W_{:,i\times50+j}$ which is the outer
product of $U_{:,i}$ and $V_{:,j}$.\label{fig:MNIST_weights}}
\end{figure}


\subsection{Autoencoders for Corrupted Face Reconstruction}

To evaluate the ability of learning structural information in images
of matrix-centric nets, we conduct experiments on the Frey Face dataset\footnote{http://www.cs.nyu.edu/\textasciitilde{}roweis/data.html},
which consists of 1,965 face images of size $28\times20$, taken from
sequential frames of a video. We randomly select 70\% data for training,
20\% for testing and 10\% for validation. Test images are corrupted
with $5\times5$ black square patches at random positions.  Auto-encoders
(AEs) are used for this reconstruction task. We build deep AEs consisting
of 20 and 40 layers. For each depth, we select vector nets with 50,
100, 200 and 500 hidden units and matrix nets with hidden shape of
$20\times20$, $50\times50$, $100\times100$ and $150\times150$.
The encoders and the decoders have tied weights.  The AEs are trained
with backprop, random noise added to the input with ratio of $0.2$,
 and L1 and L2 regularizers. 

\begin{figure*}
\begin{centering}
\subfloat[\label{fig:FreyFace_a}]{\begin{centering}
\begin{tabular}{c}
\includegraphics[height=0.33\textwidth]{FreyFace-test_x}\includegraphics[height=0.33\textwidth]{FreyFace-test_y}\tabularnewline
\end{tabular}
\par\end{centering}
}~~~\subfloat[\label{fig:FreyFace_b}]{\begin{centering}
\begin{tabular}{c}
\includegraphics[height=0.33\textwidth]{FreyFace-vec-d20-h50}\includegraphics[height=0.33\textwidth]{FreyFace-vec-d20-h500}\tabularnewline
\end{tabular}
\par\end{centering}
}~~~\subfloat[\label{fig:FreyFace_c}]{\begin{centering}
\begin{tabular}{c}
\includegraphics[height=0.33\textwidth]{FreyFace-vec-reg}\tabularnewline
\end{tabular}
\par\end{centering}
}~~~\subfloat[\label{fig:FreyFace_d}]{\begin{centering}
\begin{tabular}{c}
\includegraphics[height=0.33\textwidth]{\string"FreyFace-mat-d20-h20,20\string".pdf}\includegraphics[height=0.33\textwidth]{\string"FreyFace-mat-d20-h50,50\string".pdf}\includegraphics[height=0.33\textwidth]{\string"FreyFace-mat-d20-h150,150\string".pdf}\tabularnewline
\end{tabular}
\par\end{centering}
}~~~\subfloat[\label{fig:FreyFace_e}]{\begin{centering}
\begin{tabular}{c}
\includegraphics[height=0.33\textwidth]{FreyFace-mat-l1}\tabularnewline
\end{tabular}
\par\end{centering}
}~~~\subfloat[\label{fig:FreyFace_f}]{\begin{centering}
\begin{tabular}{c}
\includegraphics[height=0.33\textwidth]{\string"FreyFace-mat-d10-h50,50-l2\string".pdf}\includegraphics[height=0.33\textwidth]{\string"FreyFace-mat-d10-h150,150-l2\string".pdf}\tabularnewline
\end{tabular}
\par\end{centering}
}
\par\end{centering}
\caption{Images reconstructed by matrix AEs and vector AEs in comparison with
ground truth. All AEs from \textbf{(b)} to \textbf{(e)} have 40 layers
while the AEs at \textbf{(f)} have 20 layers.\textbf{ (a):} corrupted
inputs and ground truth; \textbf{(b):} vector AEs (hidden size of
$50$ and $500$) without regularization; \textbf{(c):} vector AEs
with regularization; \textbf{(d):} matrix AEs (hidden size of $20\times20$,
$50\times50$ and $150\times150$) without regularization; \textbf{(e):}
matrix AEs with L1 regularization; \textbf{(f):} matrix AEs (hidden
size of $50\times50$ and $150\times150$) with L2 regularization.\label{fig:FreyFace_rec} }
\end{figure*}

Once trained, AEs are used to reconstruct the test images. Fig.~\ref{fig:FreyFace_rec}
presents several reconstruction results. Vector AEs fail to learn
to reconstruct either with or without weight regularization. Without
weight regularization, vector AEs fail to remove noise from the training
images (Fig.~\ref{fig:FreyFace_b}), while with weight regularization
they collapse to a single mode (Fig.~\ref{fig:FreyFace_b})\footnote{This happens for all hidden sizes and all depth values of vector AEs
specified above.}. Matrix AEs, in contrast, can reconstruct the test images quite well
\emph{without weight regularization} (see Fig.~\ref{fig:FreyFace_d}).
In fact, adding weight regularization to matrix AEs actually deteriorates
the performance, as shown in Figs.~\ref{fig:FreyFace_rec}(e,f).
This suggests a couple of conjectures. One is there exists structural
regularization in matrix-centric nets (e.g., due to the implicit weight
matrix-factorization shown in Section.~\ref{subsec:Low-rank}), hence
weight regularization is not needed. The other is that matrix-like
structures in images are preserved in matrix-centric nets, enabling
missing information to be recovered.


\subsection{Sequence to Sequence Learning with Moving MNIST}

In this experiment, we compare the performance of matrix and vector
recurrent nets in a \emph{sequence-to-sequence} (seq2seq) learning
task \cite{sutskever2014sequence,srivastava2015unsupervised}. We
choose the Moving MNIST dataset\footnote{http://www.cs.toronto.edu/\textasciitilde{}nitish/unsupervised\_video/}
which contains 10K image sequences. Each sequence has length of 20
showing 2 digits moving in $64\times64$ frames. We randomly divide
the dataset into 6K, 3K and 1K image sequences with respect to training,
testing and validation. In our seq2seq model, the encoder and the
decoder are both recurrent nets. The encoder captures information
of the first 15 frames while the decoder predicts the last 5 frames
using the hidden context learnt by the encoder. Different from \cite{srivastava2015unsupervised},
the decoder do not have readout connections\footnote{the predicted output of the decoder at one time step will be used
as input at the next time step} for simplicity. We build vector seq2seq models with hidden sizes
ranging from $100$ to $2000$ for both the encoder and the decoder.
In case of matrix seq2seq models, we choose hidden sizes from from
$10\times10$ to $200\times200$. Later in this section, we write
vector RNN/LSTM to refer to a vector seq2seq model with the encoder
and decoder are RNNs/LSTMs. The same notation applies to matrix.

\begin{figure}[t]
\begin{centering}
\includegraphics[width=0.9\columnwidth]{MovingMNIST_loss}
\par\end{centering}
\caption{Reconstruction loss over test data of matrix and vector seq2seq models
as functions of hidden unit. \emph{DO} is short for Dropout which
is set at 0.2 for inputs and 0.5 for hidden units. Best viewed in
color.\label{fig:MovingMNIST_plot}}
\end{figure}

It is important to emphasize that matrix-centric nets are far more
compact than the vector-centric counterparts. For example, the vector
RNNs require nearly 30M parameters for 2K hidden units while the matrix
RNNs only need about 400K parameters (roughly 75 times fewer) but
have 40K hidden units (20 times larger)\footnote{For LSTMs, the number of parameters quadruples but the relative compactness
between vector and matrix-centric nets remain the same.}. The parameter inflation exhibits a huge redundancy in vector representation
which makes the vector nets susceptible to overfitting. Therefore,
after a certain threshold (200 in this case), increasing the hidden
size of a vector RNN/LSTM will deteriorate its performance. Matrix
nets, in contrast, are consistently better when the hidden shape becomes
larger, suggesting that overfitting is not a problem. Remarkably,
a matrix RNN/LSTM with hidden shape of $50\times50$ is enough to
outperform vector RNNs/LSTMs of any size with or without dropout (see
Fig.~\ref{fig:MovingMNIST_plot}). Dropout does improve the representations
of both vector and matrix nets but it cannot eliminate the overfitting
on the big vector nets.


\subsection{Sequence Classification with EEG}

We use the Alcoholic EEG dataset\footnote{https://kdd.ics.uci.edu/databases/eeg/eeg.data.html}
of 122 subjects divided into two groups: alcoholic and control groups.
Each subject completed about 100 trials and the data contains about
12K trials in total. For each trial, the subject was presented with
three different types of stimuli in $1$ second. EEG signals have
64 channels sampled at the rate of 256 Hz. Thus, each trial consists
of $64\times256$ samples in total. We convert the signals into spectrograms
using Short-Time Fourier Transform (STFT) with Hamming window of length
$64$ and $56$ overlapping samples. The signals were detrended by
removing mean values along the time axis. Because the signals are
real-valued, we only take half of the frequency bins. We also exclude
the first bin which corresponds to zero frequency. This results in
a tensor of shape $64\times32\times25$ where the dimensions are channel,
frequency and time, respectively. Fig.~\ref{fig:EEG_Spec} shows
examples of the input spectrogram of an alcoholic subject in 4 channels
which reveals some spatial correlations across channels and frequencies.
For this dataset, we randomly separate the trials of each subject
with a proportion of 0.6/0.2/0.2 for training/testing/validation.

\begin{figure}
\begin{centering}
\includegraphics[scale=0.24]{EEG_4_channels}
\par\end{centering}
\caption{Spectrograms of four channels taken from one trial of a random alcoholic
subject. Best viewed in color.\label{fig:EEG_Spec}}
\end{figure}

To model the frequency change of all channels over time, we use LSTMs
\cite{hochreiter1997long}. We choose vector LSTMs with 200 hidden
units which show to work best in the experiment with Moving MNIST.
For matrix LSTMs, we select the one with hidden shape of $100\times100$.
We evaluate six different settings for this task. Models 1 and 2 both
receive plain spectrogram inputs which are sequences of matrices of
shape $64\times32$. In case of Model 1, these matrices are flattened
into vectors. Models 3, 4, 5, 6 use an additional spatial feature
detector which is a 2-conv (short for convolutional) layer CNN. The
first conv layer uses $32$ filters of shape $5\times5$ while the
second conv layer uses $64$ filters of shape $3\times3$. Each conv
layer is followed by a $2\times2$ subsampling layer. Hence, the output
of this CNN model is a tensor of shape $64\times14\times6$. For Model
3, we add a global conv layer (denoted as \emph{CNN-g} in Tab.~\ref{tab:EEG_result})
with 200 filters of shape $14\times6$ above the CNN and get an output
vector of length $200$. We feed this vector to the vector LSTM. For
Model 5, we reshape the $64\times14\times6$ tensor into a $64\times84$
matrix (\emph{CNN-s}) and feed it to the matrix LSTM. Models 4 and
6 employ the tensor-matrix mapping described in Section.~\ref{subsec:Tensor-Matrix-Mapping}
to convert this tensor into a matrix of shape $50\times50$ (\emph{CNN-m}),
which is fed to the vector LSTM (after vectorization) and the matrix
LSTM, respectively.  

As seen in Tab.~\ref{tab:EEG_result}, the vector LSTM with raw input
(Model 1) not only achieves the worst result but also consumes a very
large number of parameters. The plain matrix LSTM (Model 2) improves
the result by a large margin (about 3.5\%) while having far fewer
parameters than of Model 1. When the CNN feature detector is presented
(in Models 3 and 4), the errors for the vector LSTMs drop dramatically,
suggesting that spatial representation is important for this type
of data. However, even with the help of conv layers, the vector LSTMs
are not able to compete against the plain matrix LSTM.

Similar to vector LSTMs, we can use the CNN to detect feature maps
for matrix LSTMs. However, if we just simply reshape the output of
the CNN as being done in Model 5, the result will be poorer. This
is because the reshaping destroys the 2D information of each feature
map. On the other hand, with proper tensor-matrix mapping (see Section~\ref{subsec:Tensor-Matrix-Mapping})
where the 2D structure is preserved, matrix LSTM (Model 6) yields
the best result of 1.44\% error, which compares favorably to the best
result achieved by the vector LSTMs (1.90\%). Importantly, this matrix
LSTM requires 6 times less parameters than its vector counterpart.

\begin{table}
\begin{centering}
\begin{tabular}{|l|r|c|}
\hline 
\emph{Model} & \emph{\# Params} & \emph{Err (\%)}\tabularnewline
\hline 
\hline 
vec-LSTM (1) & 1,844,201 & 5.29\tabularnewline
mat-LSTM (2) & 160,601 & 1.71\tabularnewline
\hline 
CNN-g + vec-LSTM (3) & 1,435,729 & 1.90\tabularnewline
CNN-m + vec-LSTM (4) & 2,266,829 & 2.63\tabularnewline
CNN-s + mat-LSTM (5) & 200,729 & 4.12\tabularnewline
\textbf{CNN-m + mat-LSTM (6)} & \textbf{248,029} & \textbf{1.44}\tabularnewline
\hline 
\end{tabular}
\par\end{centering}
\caption{Classification accuracy and number of parameters of different models.
\emph{CNN-g}: global vectorization of CNN output, \emph{CNN-m}: tensor-matrix
mapping of CNN output, \emph{CNN-s} = simple reshaping by vectorization
per channel of the CNN output. \label{tab:EEG_result}}
\end{table}



==> matrix-intro-v3_sv.tex <==
Recent advances in deep learning have generated a constant stream
of new neural architectures, ranging from variants of feed-forward
nets to differentiable Turing machines \cite{lecun2015deep,graves2016hybrid}.
Nevertheless, the central components of these nets are still reliant
on vector representations due to simplicity in mathematical modeling
and programming. For domains where data are naturally represented
in matrices, for example, images or multi-channel signals, the vector
representation is sub-optimal because of two reasons. First, it requires
vectorization by stretching all columns into a single vector \textendash{}
this operation destroys the intrinsic multi-mode structure. Second,
failing to account for the relations between data modes usually leads
to a larger model whose parameters grow with the number of matrix
cells.

To overcome these drawbacks, we present a new notion of distributed
representation for matrix data wherein the input, hidden and output
layers are matrices. The connection between an input and an output
layer is a nonlinear\textit{ matrix-matrix mapping} parameterized
by two other parameter matrices, one that captures the correlation
between rows, and the other captures the correlation between columns.
\textit{\emph{It results in}}\emph{ a powerful yet highly compact
model that is not only able to represent the structure of a matrix
but also has a parameter growth rate that equals the largest dimension
of the matrix.}\textit{\emph{ }}

\textit{\emph{We have discovered an attractive feature of the matrix-matrix
mapping in that it allows us to build deep matrix networks, circumventing
this problem with equivalent vector representations.}}\emph{ }\textit{\emph{It
acts as a kind of regularization to the matrix structure, and we term
it}}\emph{ structural regularization}\textit{\emph{.}} \textit{\emph{Furthermore,}}
all neural networks that use conventional vector representations can
be replaced with the matrix counterparts we propose, creating new
matrix-centric neural nets. We demonstrate the application of our
techniques for feed-forward networks, recurrent networks and finally
convolutional networks. For recurrent nets, each time step has a matrix
memory where rows/columns can be considered as memory slots and matrix
mapping works like the attentive reading operator in \cite{graves2014neural}.
Convolutional nets \cite{lecun1995convolutional} whose output is
typically a set of 2D feature maps can be combined seamlessly with
matrix-centric networks using \textit{\emph{tensor-matrix mapping}},
and this preserves spatial structure of feature maps.

We evaluate our methods on four diverse experiments. The first uses
feed-forward nets for handwritten digit recognition. The second problem
is face reconstruction from occlusion using auto-encoders. In these
two experiments, we carefully examine the structural regularization
effect. Next is a sequence-to-sequence learning task wherein we test
the performance of matrix recurrent nets. Finally, for classification
of EEG signals, we integrate CNNs used as feature extractors with
matrix LSTMs to model the temporal dynamics of frequencies along different
channels.

To summarize, our main contributions are:
\begin{itemize}
\item Introduction of a novel neural net approach that incorporates matrices
as the basic representation;
\item Hypothesis about a regularization mechanism related to the matrix
mapping for such architectures;
\item Derivation of new matrix representation alternative for the two canonical
architectures:\textit{ }\textit{\emph{feed-forward nets}} and \textit{\emph{recurrent
nets}}. We also propose a method to convert the output of convolutional
layers into a matrix, which can then be used in matrix feed-forward
nets or recurrent nets;
\item Demonstration of the efficacy of matrix-centric neural nets on a comprehensive
suite of experiments.
\end{itemize}



==> matrix-method-v2.tex <==
We present our main contribution, the matrix-centric neural architectures.

\subsection{Matrix-Matrix Mapping}

With conventional vector representation, the mapping from an input
vector $\xb$ to an output vector $\yb$ has the form $\yb=\sigma(W\xb+\bb)$
where $\bb$ is a bias vector, $W$ is a mapping matrix and $\sigma$
is an element-wise nonlinear transformation.

Likewise, in our new matrix representation, the building block is
a mapping from an input matrix $X$ of size $c_{1}\times r_{1}$ to
an output matrix $Y$ of size $c_{2}\times r_{2}$, as follows:

\begin{eqnarray}
Y & = & \sigma(U^{\intercal}XV+B)\label{eq:matrix_mapping}
\end{eqnarray}
where $U\in\Real^{c_{1}\times c_{2}}$ is the \textit{row mapping}
matrix, $V\in\Real^{r_{1}\times r_{2}}$ is the \textit{column mapping}
matrix and $B\in\Real^{c_{2}\times r_{2}}$ is the bias matrix. With
this mapping, building a deep feedforward network is straightforward
by stacking the matrix-matrix layers on top of each other.

Eq.~(\ref{eq:matrix_mapping}) has interesting properties. First,
the number of parameter scales linearly with only the largest dimension
of input/output matrices with $c_{1}c_{2}+r_{1}r_{2}+c_{2}r_{2}$
parameters. For conventional vector representation, we would need
$c_{1}c_{2}r_{1}r_{2}+c_{2}r_{2}$ parameters. Second, the representation
in Eq.~(\ref{eq:matrix_mapping}) is indeed a low-rank factorization
of the mapping matrix in the case of full vector representation, which
we will show next. 

\subsection{Matrix-Matrix Mapping as Low-Rank Factorization\label{subsec:Low-rank}}

Assume that we vectorize $X$ and $Y$ into vector $\xb$ of length
$c_{1}r_{1}$ and $\yb$ of length $c_{2}r_{2}$, respectively and
use standard vector-vector mapping between them: $\yb=\sigma(W^{\intercal}\xb+b)$
where $W$ is the parameter matrix of shape $c_{1}r_{1}\times c_{2}r_{2}$.
Thus, each element $y_{k}$ with $k\in\{1,...,c_{2}r_{2}\}$ can be
computed as follows:

\begin{eqnarray}
y_{k} & = & \sigma\left(W_{:,k}^{\intercal}\xb+b_{k}\right)\nonumber \\
 & = & \sigma\left(\sum_{\text{all elements}}(W_{:,k}\odot\xb)+b_{k}\right)\label{eq:vector_odot}
\end{eqnarray}

On the other hand, we can slightly modify Eq.~(\ref{eq:matrix_mapping})
to describe the mapping from the entire matrix $X$ to an element
$Y_{i,j}$ of the matrix $Y$:

\begin{eqnarray}
Y_{i,j} & = & \sigma\left(U_{:,i}^{\intercal}XV_{:,j}+B_{ij}\right)\nonumber \\
 & = & \sigma\left(\sum_{\text{all elements}}(U_{:,i}V_{:,j}^{\intercal}\odot X)+B_{ij}\right)\label{eq:matrix_odot}
\end{eqnarray}

If we refer $y_{\ensuremath{k}}$ and $Y_{i,j}$ to be the same component,
e.g. $k=i\times r_{2}+j$, Eq.~(\ref{eq:vector_odot}) and Eq.~(\ref{eq:matrix_odot})
must be equal. Then we have:

\begin{eqnarray}
\text{matrix}(W_{:,i\times r_{2}+j}) & = & U_{:,i}V_{:,j}^{\intercal}\label{eq:low_rank}
\end{eqnarray}
where $\text{matrix}(W_{\ensuremath{;i\times r_{2}}+j})$ means that
the column vector $W_{\ensuremath{;i\times r_{2}}+j}$ of length $c_{1}r_{1}$
is reshaped to a matrix of shape $c_{1}\times r_{1}$. Eq.~(\ref{eq:low_rank})
shows that the weights $U_{:,i}$ and $V_{:,j}$ that map the whole
input matrix $X$ to an output element $Y_{\ensuremath{i,j}}$ is
the low-rank decomposition of the dense weights $W_{:,i\times r_{2}+j}$
used in equivalent vector mapping. .

\subsection{Matrix Recurrent Networks}

We now present the matrix extension of recurrent networks. Here, the
input, output and hidden state at each time step are matrices. For
ease of development, let us introduce the notation $\mat(X,H;\thetab)$,
defined as:

\begin{eqnarray}
\mat(X,H;\thetab) & := & U_{x}^{\intercal}XV_{x}+U_{h}^{\intercal}HV_{h}+B\label{eq:mat_mapping_LSTM}
\end{eqnarray}
where $\thetab=\{U_{x},V_{x},U_{h},V_{h},B\}$. The next state in
vanilla matrix-RNNs is simply:

\[
H_{t}=\sigma\left(\mat\left(X_{t},H_{t-1};\thetab_{i}\right)\right)
\]

In case of matrix Long Short-Term Memory (matrix-LSTM), the formula
of a block (without peep-hole connection) at time step $t$ can be
specified as follows:

\begin{eqnarray*}
I_{t} & = & \sigma(\mat(X_{t},H_{t-1};\thetab_{i}))\\
F_{t} & = & \sigma(\mat(X_{t},H_{t-1};\thetab_{f}))\\
O_{t} & = & \sigma(\mat(X_{t},H_{t-1};\thetab_{o}))\\
\hat{C_{t}} & = & \tanh(\mat(X_{t},H_{t-1};\thetab_{c}))\\
C_{t} & = & F_{t}\odot C_{t-1}+I_{t}\odot\hat{C}_{t}\\
H_{t} & = & O_{t}\odot\tanh(C_{t})
\end{eqnarray*}
where $\odot$ denotes the Hadamard product; and $I_{t}$, $F_{t}$
$O_{t}$, $\hat{C_{t}}$ are input gate, forget gate, output gate
and cell gate at time $t$, respectively. Note that the memory cells
$C_{t}$ that store, forget and update information is a matrix.

\paragraph{Remark:}

The second term $U_{h}^{\intercal}HV_{h}$ in Eq.~(\ref{eq:mat_mapping_LSTM})
bears some similarity with the external memory bank in a Neural Turing
Machine \cite{graves2014neural,graves2016hybrid}. The state matrix
$H$ can be viewed as an array of memory slots while each $i$-th
column vector of the matrix $U_{h}^{\intercal}$ acts as (unnormalized)
attention weights to select which rows of $H$ to read from and each
$j$-th row of the matrix $V_{h}$ specifies which parts of a memory
slot are most informative.

\subsection{Tensor-Matrix Mapping \label{subsec:Tensor-Matrix-Mapping}}

For spatial inputs, convolutional layers are essential to learn translation-invariant
features. The output of a convolutional layer is usually a set of
2D feature maps \textendash{} or in other words, a 3D tensor.  The
matrix neural nets defined above can easily connect to CNNs using
a \emph{tensor-matrix mapping}. Since these feature maps are structured,
flattening them into vectors as in conventional CNNs may loose information.
We propose to treat these 2D maps as matrices. 

Denote $\Xcal$ as the output of the convolutional layer. $\Xcal$
is a 3D tensor of shape $(m,c_{1},r_{1})$ where $m$ is the number
of feature maps, each has shape $c_{1}\times r_{1}$. We want to map
this tensor to a 2D matrix $Y$ of shape $(c_{2},r_{2})$. To do so,
we use two 3D tensors $\Ucal$ and $\Vcal$ of shape $(m,c_{1},c_{2})$
and $(m,r_{1},r_{2})$ respectively as parameters. Then the tensor-matrix
mapping is defined as:

\begin{eqnarray}
Y & = & \sum_{i=1}^{m}\Ucal_{i}^{\intercal}\Xcal_{i}\Vcal_{i}\label{eq:conv_matrix_map}
\end{eqnarray}
See Fig.~\ref{fig:Convolution-matrix-mapping} for a graphical illustration.
 With this mapping, CNNs can naturally serve as a feature detector
for matrix-centric neural nets in spatial domains.

\begin{figure}
\begin{centering}
\includegraphics[scale=0.23]{CNN_matrix_mapping}
\par\end{centering}
\caption{Tensor-matrix mapping, where $\protect\Xcal$ is the tensor output
of the convolutional layer, $Y$ is the desired matrix representation,
and $\left\{ \protect\Ucal_{i},\protect\Vcal_{i}\right\} _{i=1}^{m}$
are mapping parameters.\label{fig:Convolution-matrix-mapping}}
\end{figure}




==> matrix-related.tex <==
Matrix data modeling has been well studied in shallow or linear settings,
such as 2DPCA \cite{yang2004two}, 2DLDA \cite{ye2004two}, Matrix-variate
Factor Analysis \cite{xie2008matrix}, Tensor analyzer \cite{tang2013tensor},
Matrix/tensor RBM \cite{nguyen2015tensor,qi2016matrix}. Except 2DPCA
and 2DLDA, all other methods are probabilistic models which  use
matrix mapping to parameterize the conditional distribution of the
observed random variable given the latent variable. However, since
these models are shallow, their applications of matrix mapping are
limited. Our work  inherits the matrix mapping idea from these models
and extends it to a wide range of deep neural networks.

There have been several original deep architectures recently proposed
to handle \emph{multidimensional data} such as Multidimensional RNNs
\cite{graves2009offline}, Grid LSTMs \cite{kalchbrenner2015grid}
and Convolutional LSTMs \cite{xingjian2015convolutional}. The main
idea of the first two models is that any spatial dimension can be
considered as a temporal dimension. They extend the standard recurrent
networks by making as many new recurrent connections as the dimensionality
of the data. These connections allow the network to create a flexible
internal representation of the surrounding context. Although Multidimensional
RNNs and Grid LSTMs are shown to work well with many high dimensional
datasets, they are complicate to implement and have a very long recurrent
loop (often equal to the input tensor's shape) run sequentially.
A convolutional LSTM, on the other hand, works like a standard recurrent
net except that its gates, memory cells and hidden states are all
3D tensors with convolution as the mapping operator. Consequently,
each local region in the hidden memory is attended and updated over
time. This is different from our model since a matrix recurrent net
attends to every row/column vector of its hidden memory.

We are also aware of another work \cite{novikov2015tensorizing} that
proposes matrix decomposition of the weight matrix in vector-vector
mapping similar to ours. They show that this kind of matrix decomposition
is, indeed, a specific case of a more general Tensor Train (TT) transformation
\cite{oseledets2011tensor} when the tensor is a 2D matrix. However,
their work solely focuses on model compression using the TT transformation
for feed-forward nets\footnote{They do use CNNs in their paper but only the top fully-connected layers
are modified with TT transformation}. Our main contributions are creating a matrix-centric ecosystem of
neural nets, which include feed-forward, recurrent and convolutional
architectures.

RNNs with augmented memory and attention present an implicit use of
matrix modeling: each row is a piece of memory and the entire memory
is a matrix (e.g., those in NTM \cite{graves2014neural,graves2016hybrid}
and Memory Networks \cite{weston2014memory}). Reading and writing
require attention to a specific memory piece. However, most attention
schemes maintain a softmax distribution over all memory pieces to
maintain differentiability. The attention distribution is like the
row-mapping matrix in our case.

